Substrate Asymmetry in User-Side Memory: A Diagnostic Framework

User-side memory in LLMs is typically scored as a single "personalization" capability: given a user's history, is the output more user-aware? We show this aggregate metric hides opposite-direction failures. Memory factorises into at least three orthogonal axes -- behavioral consistency (style, voice), factual presence (recall facts in history), and factual absence (abstain when a fact is absent) -- and no single substrate wins all three. Comparing per-user gamma-LoRA (a small LoRA adapter trained on each user's history; gamma denotes per-user, not per-task) against BGE-large dense top-K retrieval on a controlled 50-user synthetic corpus and a real-data probe (LaMP-3), we find gamma-LoRA decisively wins behavioral style while RAG decisively wins factual absence -- and the same query-projection cells in attention layers 21-35 causally load-bear both effects in opposite directions (zeroing those LoRA weights raises absence-probe TPR by +33 pp and drops presence-probe TPR by 20 pp). On the more heavily RLHF-tuned Llama-3.1-8B-Instruct the asymmetry strengthens, not heals: parametric memory's behavioral advantage collapses while its absence-calibration deficit against retrieval widens -- an alignment tax on parametric user-memory. On real-data LaMP-3, gamma-LoRA underperforms a majority baseline; a 9-condition mitigation sweep diagnoses this as instruction-following collapse, not substrate failure (a 9x2 cross-product shows the eval-time {1..5} logit mask drives main_acc to >=0.995 on every recipe), and the best training-time fix replicates bit-identically on Llama. Finally, substrate-selection routing is question-classification, not calibration: a 110M DistilBERT on the question text alone beats every logit-based router. We contribute the diagnostic framework, the diagnosed real-data negative, the alignment-tax replication, and the routing-as-classification finding.

==> sections/conclusion.tex <==
\section{Conclusion}\label{conclusion}

User-side memory in LLMs is not one capability but a small number of
separable ones. Our framework --- three axes (behavioral, presence,
absence), two corpora (synthetic, LaMP-3), two substrates (γ-LoRA,
BGE) --- makes the separation measurable. Synthetic substrates split
cleanly (γ-LoRA +0.473 nat/tok, 59.8\% LLM-judge at n=750; RAG +45.7pp absence;
same q\_proj L21--35 band drives both, opposite directions). On
LaMP-3 the asymmetry does not transfer (31.5\% vs majority 59.5\%)
but is \emph{diagnosed} in §4.3.6: an eval-time logit mask drives
main\_acc to ≥0.995 on every one of 8 training recipes (cross-product
robustness), isolating instruction-following collapse from substrate
failure; both eval-time and training-time fixes replicate on
Llama-3.1-8B. On Llama, calibration asymmetry strengthens (+79pp)
but style collapses --- qualitative pattern travels, magnitudes are
model-specific. Hybrid-routing pre-registered (Appendix D);
limitations in §6.

